Physics-constrained machine learning for thermal turbulence modelling at low Prandtl numbers

Liquid metals play a central role in new generation liquid metal cooled nuclear reactors, for which numerical investigations require the use of appropriate thermal turbulence models for low Prandtl number fluids. Given the limitations of traditional modelling approaches and the increasing availability of high-fidelity data for this class of fluids, we propose a Machine Learning strategy for the modelling of the turbulent heat flux. A comprehensive algebraic mathematical structure is derived and physical constraints are imposed to ensure attractive properties promoting applicability, robustness and stability. The closure coefficients of the model are predicted by an Artificial Neural Network (ANN) which is trained with DNS data at different Prandtl numbers. The validity of the approach was verified through a priori and a posteriori validation for two and three-dimensional liquid metal flows. The model provides a complete vectorial representation of the turbulent heat flux and the predictions fit the DNS data in a wide range of Prandtl numbers (Pr=0.01-0.71). The comparison with other existing thermal models shows that the methodology is very promising.

==> Sections/Introduction_old <==
Liquid metal heat transfer underlies many phenomena and engineering applications. Steel production, the development of liquid metal batteries and new generation solar power systems and the cooling of fission nuclear reactors are examples of problems requiring the understanding of liquid metal thermal hydraulics. Such fluids are indeed very attractive for problems of huge heat removal, due to their high thermal conductivity, small vapour pressure and the wide temperature range over which they remain in liquid state. Many of the applications of interest require the accurate design and optimisation of heat transfer systems, which need a complete analysis of the thermal hydraulics conditions establishing during normal operations and transients. \\
Nowadays, a so detailed analysis of the thermal field is definitely challenging. From an experimental point of view, the opacity of liquid metals makes measurements considerably hard. The numerical approach is problematic as well, since most of the relevant liquid metal flows are turbulent. The Direct Numerical Simulation (DNS) and the Large Eddy Simulation (LES) of turbulence are impractical in most of the scenarios of industrial interest, due to the high Reynolds or Grashof numbers involved and the amount of geometrical details characterizing the flow domains. The Reynolds Averaged Navier-Stokes (RANS) approach appears then as the only feasible choice to obtain a full description of the thermal field with reasonable computational costs.


In a RANS framework, the governing equations for such incompressible, non-isothermal flows can be written as:
\begin{linenomath}
\begin{equation}
    \frac{\partial U_i}{\partial t}+ U_j \frac{\partial U_i}{\partial x_j} = -\frac{1}{\rho} \frac{\partial P}{\partial x_i} - \frac{\partial \overline{u_i u_j}}{\partial x_j} + \beta g_i \left(T-T_0 \right) +\nu \frac{\partial^2 U_i}{\partial{x_j}\partial x_j}
\label{mean_flow}
\end{equation}
\end{linenomath}
\begin{linenomath}
\begin{equation}
\begin{split}
\frac{\partial T}{\partial{t}}+U_j\frac{\partial T}{\partial{x_j}}=\alpha \frac{\partial^2 T}{\partial{x_j}\partial x_j}- \frac{\partial  \overline{u_j \theta}}{\partial{x_j}} 
\end{split}
\label{temp}
\end{equation}
\end{linenomath}
where the Boussinesq approximation is generally accepted for these flows in presence of considerable buoyancy effects. When the buoyancy contribution is negligible, 
the velocity field is independent of the temperature that can be then considered as a passive scalar of the flow. \\
Eq. \eqref{mean_flow} and \eqref{temp} introduce two unclosed statistics $\overline{u_i u_j}$ and $\overline{u_i \theta}$ that need to be modelled to solve both momentum and energy equations. The modelling of the Reynolds Stress Tensor $\overline{u_i u_j}$ is a typical problem in turbulence modelling, which has been the focus of fluid mechanics research for decades. The modelling of the turbulent heat flux is a more recent topic of increasing interest, as in most of the practical applications turbulent convection is much more important than conduction. The thermal turbulence modelling is then a key point of heat transfer research to retrieve the correct thermal field and obtain reliable predictions. \\
A thermal RANS model aims at expressing the turbulent heat flux $\overline{u_i \theta}$ as a function of the other thermal and momentum statistics. This quantity in general depends on the entire history of the momentum and thermal fields over the whole domain of interest:
\begin{linenomath}
\begin{equation}
    \overline{u_i \theta} (x,t)= \mathscr{F}_i \left[\bm{U}(y,s),\bm{u}(y,s),T(y,s),\theta(y,s)\right] (x,t) \text{ for } y\in V \text{ , } s \in (0,t)
\label{problem}
\end{equation}
\end{linenomath}
The ansatz introduced by eq.\eqref{problem} can be considerably simplified if approximations based on similarity arguments are applied to model $\overline{u_i \theta}$. Similarity hypothesis were widely used in the past, and they still represent the usual engineering practice in presence of common fluids as water or air. The direct analogy between thermal and momentum fields reduces the modelling of the turbulent heat flux to the modelling of the Reynolds stresses, thus lowering the modelling efforts. 
Nevertheless, the low Prandtl numbers of liquid metals seem to undermine the similarity between momentum and thermal boundary layers. Figure \ref{dns_channel} shows the thermal and momentum fields resulting from an LES simulation at low Prandtl number: the thermal boundary layer is much thicker than the momentum one as a consequence of the high conductivity. As a result of that, there will be no perfect correspondence between momentum and thermal logarithmic layers, which is the basis of the similarity assumption. 
This consideration explains why similarity approaches (e.g. Reynolds analogy) need to be carefully reassessed at low Prandtl numbers, as also the limitations that these simple models showed in several analysis  \cite{de2018influence,shams2019towards,de2018application}.  \\
More sophisticated models were then introduced to overcome the limitations of similarity approaches. In this paper we give an overview of the available thermal turbulence models, with special attention to their applicability at low Prandtl numbers. Thermal models for the eddy diffusivity are presented in section (). These models are aimed at defining a proportionality factor describing the turbulent transport of thermal energy. Algebraic closures for $\overline{u_i \theta}$ provide a more complete vectorial representation of the turbulent heat flux, although the approach is still local by definition. This category of thermal turbulence model is discussed in detail in section ().  The most detailed approach to model $\overline{u_i \theta}$ is represented by second order closure models, which introduce evolutionary equations for the turbulent heat flux. These models are described in the last section. \\
The mentioned approaches are common in RANS modelling and were widely chosen to model the Reynolds stresses with a remarkable level of accuracy. Hence, their extention to thermal turbulence would appear natural at first. Nevertheless, some peculiarities characterize low Prandtl number fluid flows and introduce theoretical/practical limitations to the effective applicability of these general modelling strategies. In what follows, these characteristics are presented and discussed with focus on their consequences in the modelling of the turbulent heat flux.  
   \begin{figure}[h!]
    \centering
            \includegraphics[scale=0.40]{figures/bl.PNG}
    \caption{Temperature and velocity distributions obtained from the large-eddy simulation of a heated channel flow \cite{bricteux2012direct} at low Prandtl number ($Pr=0.01$).}
    \label{dns_channel}%% label for entire figure
\end{figure}

\subsection{Enhanced diffusion and locality assumption}
The high molecular diffusivity ($\alpha$) of liquid metals compared to their molecular viscosity ($\nu$) leads to important diffusion effects in the dynamics of the thermal fluctuations. This means that a thermal perturbation $\theta$ is further diffused than a velocity fluctuation $v$. Diffusion acts as a filter for thermal turbulence, suppressing high wavenumber fluctuations and creating large coherent structures that dominate the turbulent heat transfer. The higher correlation lenghts of thermal eddies clearly lead to significant non-locale effects related to the diffusive transport. The result of this process is a more isotropic thermal turbulence: for a heated channel flow at low Prandtl number \cite{kawamura2000dns}, the turbulent heat flux components are smaller and the streamwise and wall normal components become less different in magnitude (Figure \ref{thf_comp}). Accordingly, the turbulent heat flux budgets show negligible redistribution terms and the enhanced dissipation balances the generation of turbulent heat flux far away from the wall (Figure \ref{budgets}). \\
Non-local, diffusive effects require a differential model to be represented properly, since the conductive flux of a thermal statistics is proportional to its spatial derivative by definition. A second order closure model providing good sub-models for the diffusive transport has then more chances to well represent these flows. If an algebraic approach is chosen instead, first and second order derivatives of the turbulent heat flux are not included anymore and the inherent locality assumption appears less justifiable in this context. This can be seen if the model presented in eq. \eqref{problem} is simplified by assuming that the evolution of the turbulent fluctuations merely sets the time-scales and the length-scales of the turbulent heat flux and defines a characteristic thermal fluctuation $\Delta \theta$. If the Galilean invariance principle and the second law of thermodynamics are also considered, eq.\eqref{problem} can be reduced to:
\begin{linenomath}
\begin{equation}
\begin{split}
    \overline{u_i \theta} (x,t)=\mathscr{F}_i  \left[\bm{U}(y,s)-\bm{U}(x,s),T(y,s)-T(x,s),l_{\theta}(y,s),\tau_{\theta}(y,s), \\ \Delta \theta (y,s) \right] (x,t)  \text{ for } y\in V \text{ , } s \in (0,t) 
    \end{split}
\end{equation}
\end{linenomath}
The variables $\bm{U}(y,s)$, $T(y,s)$,$l_{\theta}(y,s)$, $\tau_{\theta}(y,s)$ and $\Delta \theta (y,s)$ can be expanded in a Taylor series around the point $(x,t)$. For example, $T(y,s)-T(x,s)$ can be written as:
\begin{linenomath}
\begin{equation}
\begin{split}
    T(y,s)-T(x,s)=(y_i-x_i) \frac{\partial T}{\partial x_i}+\frac{(y_i-x_i)(y_j-x_j)}{2} \frac{\partial^2 T}{\partial x_i \partial x_j} \\ + (s-t)(y_i - x_i) \frac{\partial^2 T}{\partial x_i \partial t} +...
    \end{split}
\end{equation}
\end{linenomath}
Only considering the dependence on the mean temperature, dimensional analysis can be applied to derive the following expression for $ \overline{u_i \theta}$:
\begin{linenomath}
\begin{equation}
  \overline{u_i \theta} (x,t)= \frac{l_{\theta}}{\tau_{\theta}} \Delta \theta \mathscr{F}_i \left[ T^*(y,s)-T^*(x,s) \right] 
\end{equation}
\end{linenomath}
where
\begin{linenomath}
\begin{equation}
\begin{split}
   T^*(y,s)-T^*(x,s)=\left[\frac{(y_i-x_i)}{l_{\theta}} \frac{\partial T}{\partial x_i} \frac{l_{\theta}}{\Delta \theta}+\frac{(s-t)}{\tau_{\theta}}\frac{(y_i-x_i)}{l_{\theta}}\frac{\partial^2 T}{\partial t \partial x_i}\frac{l_{\theta} \tau_{\theta}}{\Delta \theta} \\ +\frac{(y_i-x_i)}{\l_{\theta}}\frac{(y_j-x_j)}{l_{\theta}}\frac{\partial^2 T}{\partial x_i \partial x_j} \frac{l_{\theta}^2}{\Delta \theta} + ...\right]
    \label{approximation2}
    \end{split}
\end{equation}
\end{linenomath}
If the characteristic length scale ($l_{\theta}$) and time scale ($\tau_{\theta}$) of the turbulent heat flux are much smaller than the mean temperature scales, the mean temperature slightly varies over a distance $l_{\theta}$ and in a time interval $\tau_{\theta}$. Hence, $y_i-x_i$ and $s-t$ can be assumed equal to $l_{\theta}$ and $\tau_{\theta}$, respectively, without considerable loss of information. Expression \eqref{approximation2} can be then localized in space and time. Also, the assumption of very small $l_{\theta}$ and $\tau_{\theta}$ allows to eliminate higher order terms in eq.\eqref{approximation2}, obtaining a simple gradient approximation of the heat flux:
\begin{linenomath}
\begin{equation}
    \overline{u_i \theta}=-\frac{l_{\theta}^2}{\tau_{\theta}}\frac{\partial T}{\partial x_i}=-\alpha_t \frac{\partial T}{\partial x_i}
\end{equation}
\end{linenomath}
Nevertheless, the assumption of complete separation of scales gradually misses its validity with the decrease of the Prandtl number, due to the larger thermal structures appearing. Hence, the locality assumption characterizing algebraic closures seems quite restrictive at low Prandtl numbers: the loss of historical and non-local effects is difficult to be artificially reproduced through algebraic products, which are always local and instantaneous. \\
%Also, the increase of the thermal diffusivity cuts-off the thermal energy spectrum at high wave numbers \cite{grotzbach2013challenges}. As the thermal dissipation moves to large scales with decreasing $Pr$, thermal turbulent statistics become much more sensitive to the values of the Reynolds number with respect to near unity Prandtl number flows, as it was also underlined by Gr{\"o}tzbach \cite{grotzbach2013challenges} (Figure \ref{maximum}). \\
  \begin{figure}[h!]
    \centering
     \subfloat[$Pr=0.71$]{%
        \label{budget1}%% label for first subfigure
            \includegraphics[width=0.5\linewidth]{figures2/thf_x_CH.eps}
    \hspace{0.02\linewidth}}
%%----start of second subfigure----
    \subfloat[$Pr=0.025$]{%
        \label{budget2}%% label for second subfigure
      \includegraphics[width=0.5\linewidth]{figures2/thf_x_BL.eps}}\\
    \caption{Streamwise and wall-normal components of the turbulent heat flux for (a) turbulent channel flow  \cite{kawamura2000dns} ($Re_{\tau}=640$, $Pr=0.71$ and 0.025) and (b) turbulent boundary layer flow \cite{li2009dns} ($Pr=0.71$ and 0.2).}
    \label{thf_comp}%% label for entire figure
\end{figure} 
   \begin{figure}[h!]
    \centering
%%----start of first subfigure----
    \subfloat[$Pr=0.71$]{%
        \label{budget1}%% label for first subfigure
            \includegraphics[width=0.5\linewidth]{figures/budget_1.eps}
    \hspace{0.02\linewidth}}
%%----start of second subfigure----
    \subfloat[$Pr=0.025$]{%
        \label{budget2}%% label for second subfigure
      \includegraphics[width=0.5\linewidth]{figures/budget_2.eps}}\\
    %\hspace{0.02\linewidth}}
    %%----start of fourth subfigure----
    %%----start of first subfigure----
    \subfloat[$Pr=0.71$]{%
        \label{budget1BL}%% label for first subfigure
            \includegraphics[width=0.5\linewidth]{figures2/budgets_BL_071.eps}
    \hspace{0.02\linewidth}}
%%----start of second subfigure----
    \subfloat[$Pr=0.025$]{%
        \label{budget2BL}%% label for second subfigure
      \includegraphics[width=0.5\linewidth]{figures2/budgets_BL_02.eps}}\\
    %\hspace{0.02\linewidth}}
    %%----start of fourth subfigure----
    \caption{Budget terms from the DNS database of Kawamura et al. \cite{kawamura2000dns} (figures \ref{budget1} and \ref{budget2}) and from the turbulent boundary layer DNS database of Li et al. \cite{li2009dns} (figures \ref{budget1BL} and \ref{budget2BL}). } %\cite{kawamura2000dns} (dashed lines) compared to those obtained by %applying eq. \ref{WE_all} (solid lines) for Pr=0.71.}
    \label{budgets}%% label for entire figure
\end{figure} 
\subsection{Difference of time scales and linearity problems}
The effect of the low Prandtl number can be also appreciated by comparing the momentum and thermal time-scales. Due to the high $\alpha/\nu$ ratio, the characteristic thermal time scale is much smaller than the momentum one (Figure \ref{tau}) as the dynamics of thermal fluctuations is damped by thermal diffusion. Hence, we have basically one field that is much more responsive with respect to the other one. \\
This consideration has important consequences. For example, let us consider to model the turbulent heat flux by means of a simple \textit{Wealth-Earning-Time} (WET) hypothesis \cite{launder1988computation}:
\begin{linenomath}
\begin{equation}
\begin{split}
\underbrace{\overline{u_i \theta}}_{\text{Turbulent heat flux}} = \underbrace{\overline{u_i u_j} \frac{\partial T}{\partial x_j}}_{\text{Generation from mean temperature gradients}} \cdot \underbrace{\tau}_{\text{Characteristic time}}
\label{wet}
\end{split}
\end{equation}
\end{linenomath}
which assumes that the turbulent heat flux is given by the product of its generation rate and the characteristic time scale. From what said about the time scale ratio, the effective time-scale to be used must be much smaller than the momentum time-scale, as the thermal field is much more responsive. Due to the absence of similarity between momentum and thermal fields, the use of a proper thermal time-scale ($k_{\theta}/\epsilon_{\theta}$), or a combined thermal-mechanical time-scale \cite{so1996explicit,nagano1996development,hattori1993analysis,abe2009turbulent}, seem to be the best choice to achieve a good fit at low Prandtl numbers. \\
Nevertheless, the introduction of a thermal or combined time-scale in eq.\eqref{wet} is against the linearity principle discussed by Pope \cite{pope1983consistent}, for which the model for the turbulent heat flux should be linear with respect to the thermal statistics. This principle should be strictly valid in case buoyancy is negligible and $T$ acts as a passive scalar, since the energy equation (eq. \eqref{temp}) becomes linear in $T$. The violation of the linearity principle did not concern much the modellers, who make a wide use of thermal and mixed timescales \cite{so1996explicit,nagano1996development,hattori1993analysis,deng2001near,torii1996new} to extend rather simple thermal models to low Prandtl numbers. Indeed, the consequences of non-linearity cannot be seen in case of simple flows where only one thermal boundary condition is imposed\footnote{In case of problems involving one thermal boundary condition (e.g. channel flows with uniform heat flux b.c. or uniform temperature b.c.), a proper adimensionalisation of the thermal variables reduces the profiles of $k_{\theta}/\epsilon_{\theta}$ to a single curve, independently of the boundary heat flux or the boundary temperature.}. These simple configurations are generally selected as benchmarks for the validation of the models, thus hiding possible non-linear effects. However, in case of superimposed thermal fields (e.g. channel flows with imposed wall-normal and span-wise thermal gradients) the superimposition principle is likely to be violated by the non-linear models. Hence, testing these non-linear closures in case of complex geometries with different combinations of thermal boundary conditions appears as a priority to check their effective validity. \\
On the other hand, the difficulty to fulfill the linearity principle seems a clear indication that the modelling strategy could be further advanced to represent these flows.  Indeed, representing the heat flux based on its local generation mechanisms, as done in eq. \eqref{wet} is an implicit assumption of locality, that is probably restrictive when the effects of diffusion are so important. \\
%Beside linearity, frame independence and form independence can be also considered important properties of a constitutive relation for the turbulent heat flux. This property is not always satisfied by the existing algebraic models \cite{de2018influence,shams2019towards,de2018application}. The practical consequence of this violation is that the resulting constitutive law is affected by the dimension of the domain and on the frame of reference chosen. Although these consequences seem tolerable for many applications of interest, they compromise the applicability of the models for arbitrary geometry and flow conditions, as the model is sensitive to the choice of a reference length or/and a reference velocity.  \\
  \begin{figure}[h!]
    \centering
            \includegraphics[scale=0.35]{figures/time_scale.eps}
    \caption{Mechanical time-scale, thermal time-scale and time scale ratio ($R$) along the height of the channel \cite{kawamura2000dns} ($Re_{\tau}=180$, $Pr=0.025$).}
    \label{tau}%% label for entire figure
\end{figure} 
\subsection{Sensitivity to the Reynolds number}
The enhanced diffusivity of liquid metals cuts off the thermal energy spectrum in the high wavenumber range. This can be clearly seen in Figure \ref{spectra1}, where the one-dimensional thermal energy spectra obtained at different Prandtl numbers are compared. The thermal dissipation moves to large scales with decreasing Prandtl numbers, thus inhibiting high wavenumber fluctuations. Due to the strong damping of high frequencies and the consequent disappearance of a wide inertial range, the energy content at low wavenumbers significantly increases with the Reynolds number, as it is schematically represented in Figure \ref{spectra2}. The result of this phenomenon is that the thermal turbulence statistics become much more sensitive to the values of the Reynolds number with respect to near unity Prandtl number flows, as it was also underlined by Gr{\"o}tzbach \cite{grotzbach2013challenges} (Figure \ref{maximum}). \\
   \begin{figure}[h!]
    \centering
%%----start of first subfigure----
    \subfloat[1-D energy spectra]{%
        \label{spectra1}%% label for first subfigure
            \includegraphics[width=0.5\linewidth]{figures/spectra.eps}
    \hspace{0.02\linewidth}}
%%----start of second subfigure----
    \subfloat[3-D energy spectra]{%
        \label{spectra2}%% label for second subfigure
      \includegraphics[width=0.5\linewidth]{figures2/spectrum.png}}\\
    %\hspace{0.02\linewidth}}
    %%----start of fourth subfigure----
    \caption{Streamwise thermal energy spectra at $Pr=0.71$ and $Pr=0.025$ (DNS data of Kawamura et al. \cite{kawamura2000dns}) (a); schematic representation of the three-dimensional thermal spectra obtained in forced channel flows at unitary and low Prandtl numbers (adapted from Gr{\"o}tzbach \cite{grotzbach2013challenges}) (b).} %\cite{kawamura2000dns} (dashed lines) compared to those obtained by %applying eq. \ref{WE_all} (solid lines) for Pr=0.71.}
    \label{re_sens}%% label for entire figure
\end{figure}
This high sensitivity of the thermal statistics to the $Re$ number of the flow must be clearly taken into account while developing models for the turbulent heat flux for low Prandtl number fluids. To this end, some authors introduced an explicit Reynolds number dependence in their algebraic models for $\overline{u_i \theta}$ \cite{de2018influence,shams2019towards,de2018application}: such models are discussed in section \ref{Implicit} in more detail. This choice considerably simplifies the calibration of a thermal model since the Reynolds number is generally defined as a global parameter of the flow. On the other hand, an explicit dependence on the Reynolds number can be unfavourable and ambiguous for complex flow configurations. Indeed, a similar model would depend on the choice of a reference length and a reference velocity, which could be difficult to define for arbitrary geometry and flow conditions. For a more sensitive definition, this strong Reynolds number dependence should be translated in terms of local flow parameters, i.e. momentum turbulence statistics which are always defined for every kind of flow. However, it is clear that this would increase the complexity of the model as well as the difficulties during calibration and the possible stability issues of the resulting mathematical formulations. 

   \begin{figure}[h!]
    \centering
%%----start of first subfigure----
    \subfloat[$\overline{\theta^2}$]{%
        \label{tt}%% label for first subfigure
            \includegraphics[width=0.5\linewidth]{figures/plot_2.eps}
    \hspace{0.02\linewidth}}
%%----start of second subfigure----
    \subfloat[$\overline{v \theta}$]{%
        \label{ww}%% label for second subfigure
      \includegraphics[width=0.5\linewidth]{figures/plot_1.eps}}\\
    %\hspace{0.02\linewidth}}
    %%----start of fourth subfigure----
    \caption{Peak values achieved by the thermal turbulence statistics at different Prandtl and Reynolds numbers \cite{tiselj2001dns,kawamura2000dns}.} %\cite{kawamura2000dns} (dashed lines) compared to those obtained by %applying eq. \ref{WE_all} (solid lines) for Pr=0.71.}
    \label{maximum}%% label for entire figure
\end{figure} 

\subsection{Buoyancy effects}

The modelling troubles become more severe when the effect of buoyancy is not negligible: in such conditions, the velocity field is no more independent of the temperature field, as indicated by eq. \eqref{mean_flow} and \eqref{temp}. Even for near unity Prandtl numbers, the presence of the buoyant force in the momentum equation breaks down the analogy between momentum and thermal fields and the limitations of simple gradient transport models emerge clearly also for simple flow configurations\footnote{The Rayleigh-Bénard convection and the differentially heated cavity problem are classical examples to highlight the limits of simple gradient transport models (e.g. Reynolds Analogy)}. Algebraic anisotropic closures for the heat flux are then more appealing for such flow conditions, although they seem still restrictive due to their implicit locality assumption. Independently of the Prandtl number, buoyancy driven flows are in fact characterized by large turbulent structures that tend to slowly evolve with time. The macroscopic effects of these organized motions are rather difficult to represent with one-point closure models \cite{hanjalic2002one} and require a time-dependent mode for an accurate description. Buoyant flows are also characterized by a transient and oscillating nature, such that the flow and the temperature fields are far from the conditions of equilibrium turbulence even at large simulated time. This suggests the need of an advanced representation for both the Reynolds stresses and the turbulent heat fluxes, accounting for turbulent transport phenomena. This absence of equilibrium also lead to the coexistence of many regimes in the same flow: stagnant, laminar, transitional and fully turbulent regions can coexist in the same flow domain depending on the orientation of the temperature gradients with respect to the gravity vector. This means that the turbulence models applied to simulate these flows should be valid at both high and low Reynolds number regimes, and that the usual assumptions applied to formulate models for fully turbulent flows would not fit in such circumstances. Appropriate low-Reynolds number models are also necessary to integrate both velocity and temperature fields in the near wall region, which is characterized by significant molecular effects. Indeed, the wall function approach is rather hard to extend to buoyant flows: velocity and temperature natural convection boundary layers are strong functions of the geometrical parameters and the thermal boundary conditions imposed, i.e. an universal scaling in the near wall region cannot be defined for these flows.  \\
Low Prandtl number fluids would exacerbate the difficulties mentioned above for natural convection scenarios. Indeed, the developed thermal structures would be even larger than in case of near unity Prandtl numbers. The developed hydrodynamic boundary layers are thickened by the thermal ones, and become more likely to undergo separation near the corners of cavities or enclosures \cite{mohamad1993modeling}, formating larger secondary circulation zones and thus increasing the modelling challenges. \\
The reciprocal interaction between temperature and momentum fields is schematized in Figure \ref{buoyancy}, which follows the representation adopted by Carteciano et al. \cite{carteciano2003validation}. The turbulent heat flux is generated by buoyancy through the term $\beta g_i \overline{\theta^2}$ indicated in eq. \eqref{thf}. Then, the turbulent heat flux affects the turbulent kinetic energy through the term $\beta g_i \overline{u_i \theta}$, which also affects the mean velocity field. The change of the velocity field results in a corresponding change of the temperature field, with the consequent change of the temperature variance $\overline{\theta^2}$. It is then clear that thermal and momentum turbulence are here more strictly related with respect to forced convection scenarios. This complex dynamics of natural and mixed convection flows makes the thermal modelling very critical for both the fields. Due to the two-ways direct interaction, the effect of the turbulent heat flux model on the other fields involved is not straightforward. Hence, from a modelling point of view, this coupling practically leads to poor predictability and possible absence of monotonicity of the results with respect to the variations of the model parameters. This clearly further complicates the formulation and the calibration of thermal models. \\
In addition, the validation of thermal models for buoyant flows at various Prandtl numbers is limited by the lack of experimental data, since the low velocities arising in natural convection flows are difficult to measure with good accuracy. High fidelity approaches as DNS or LES are instead rather expensive, due to the large averaging intervals required to retrieve the values of the statistics and the need of simulating wide computational domains to capture the largest convective structures. For each Prandtl number, a complete simulation of both the thermal and momentum fields must be carried out due to the coupling of the transport equations. Also, an increase of the frequency range of the velocity fluctuations was detected in natural convection at low Prandtl numbers. This clearly increases the computational costs required by DNS and LES and imposes limits to the maximum Reynolds and Grashof numbers that can be simulated. 
  \begin{figure}[h!]
    \centering
            \includegraphics[scale=0.6]{figures/scheme_buoyancy.png}
    \caption{Rapresentation of the mechanism by which buoyancy affects both momentum and thermal fields (adapted from Carteciano et al. \cite{carteciano2003validation}). Depending on the thermal and momentum models applied to study the buoyant flow, the number of mutual dependencies between thermal and momentum fields can be either higher or lower.}
    \label{buoyancy}%% label for entire figure
\end{figure}



%and temperature and momentum fields influence each other. Indeed, independently of the Prandtl number, buoyancy driven flows are characterized by large turbulent structures that make difficult to develop consistent one-point closures \cite{hanjalic2002one}. The departure from conditions of local equilibrium turbulence, as in case of low Prandtl numbers, requires more advanced representation that also involve turbulent transport processes. This absence of equilibrium also lead to the coexistence of many regimes in the same flow: stagnant, laminar and turbulent zones could appear depending on the orientation of the temperature gradient with respect to the gravity vector. Therefore, the usual assumptions applied to formulate models for fully turbulent flows would not fit in such circumstances. Apart from that, the validation of these models is also troublesome, due to the lack of experimental data, since the low velocities arising in natural convection flows are difficult to measure with good accuracy. High fidelity approaches as DNS or LES are instead rather expensive, due to the large averaging intervals required to retrieve the values of the statistics and the need of simulating wide computational domains to capture the largest convective structures. As at low $Pr$ the span of turbulent fluctuation frequencies increases,  the computational costs become even more impressive. \\
 


%in this case, and that very accurate models for both momentum and thermal fields are required for buoyant flows, independently of the Prandtl number. Indeed, in forced convection cases we can ideally identify a very small value of $Pr$ below which the turbulent heat flux is negligible compared to the conductive flux, and the temperature distributions are minimally affected by thermal turbulence. However, this is hard to say in case of buoyant flows, where the turbulent heat flux is linked to all the variables involved. \\

\subsection{Weak and full equilibrium assumptions}
The mathematical modelling of the turbulent heat flux usually starts from the analysis of its transport equation:
\begin{linenomath}
\begin{equation}
\begin{split}
\frac{\partial{\overline{u_i \theta}}}{\partial{t}}+U_j\frac{\partial{\overline{u_i \theta}}}{\partial{x_j}}=\underbrace{\frac{\partial{}}{\partial{x_j}} \left(\nu \overline{\theta \frac{\partial{u_i}}{\partial{x_j}}}+\alpha \overline{u_i \frac{\partial{\theta}}{\partial{x_j}}} -\overline{u_i u_j \theta}  \right)}_{D_{\theta i}+T_{\theta i}} \\
\underbrace{-\overline{u_j \theta} \frac{\partial{U_i}}{\partial{x_j}}-\overline{u_i u_j} \frac{\partial{T}}{\partial{x_j}}-\beta g_i \overline{\theta^2}}_{P_{\theta i}}  \underbrace{-\overline{(\alpha+\nu)\frac{\partial{\theta}}{\partial{x_j}}\frac{\partial{u_i}}{\partial{x_j}}}}_{\epsilon_{\theta i}}+\underbrace{\overline{\theta \frac{\partial{p}}{\partial{x_j}}}}_{\psi_{\theta i}}
\label{thf}
\end{split}
\end{equation}
\end{linenomath}
where convection, molecular diffusion ($D_{\theta i}$), turbulent diffusion ($T_{\theta i}$), production ($P_{\theta i}$), dissipation  ($\epsilon_{\theta i}$) and redistribution ($\phi_{\theta i}$) correspond to different physical phenomena. The development of second order closure models is based on the modelling of transport and redistribution terms for which many models were proposed \cite{shih1990second,lumley1979computational,shin2008elliptic,dakos1987modelling}. In practical engineering applications, second order closures are generally too expensive, especially because they should to be used in combination with second order models for the Reynolds stress tensor to keep their accuracy\footnote{As the accuracy of thermal models is primarily subjected to the accuracy of computed momentum turbulence statistics, the choice of a thermal second order closure combined with a first order closure for the momentum is very uncommon.}, increasing the number of equations to be solved to 18\footnote{Specifically, 6 transport equations would be needed for the components of the Reynolds stress tensor, plus one for the dissipation rate ($\epsilon$). In addition, the thermal field would require 3 transport equations for the turbulent heat flux components, one equation for the thermal variance and one for the thermal dissipation rate ($\epsilon_{\theta}$). If these transport equations for second order statistics are added to continuity, mean velocity and energy equations, this brings the number of transport equations to solve to 18.}. Algebraic models are able to reduce the computational cost: however, they require the conversion of a differential model (eq. \eqref{thf}) into an algebraic one, with the consequent loss of non-local and historical effects, as explained above. The most utilized approach to achieve this differential-algebraic transformation is the assumption of \textit{full equilibrium} (eq.\eqref{FE}) or \textit{weak equilibrium} (eq.\eqref{WE_all}). In particular, the hypothesis of full equilibrium states that eq.\eqref{thf} can be reduced to a balance between production, redistribution and dissipation terms:
\begin{linenomath}
\begin{equation}
    P_{\theta i} + \phi_{\theta i} - \epsilon_{\theta i}=0
    \label{FE}
\end{equation}
\end{linenomath}
The weak equilibrium assumes that the that $\overline{u_i \theta}$ is almost perfectly correlated with both $\overline{\theta^2}$ and $k$, such that the following approximation for the time derivative can be considered:
\begin{linenomath}
\begin{equation}
\begin{split}
    \frac{D\overline{u_i \theta}}{Dt}= \frac{\overline{u_i \theta}}{k} \frac{D k}{Dt} \frac{1}{2} + \frac{\overline{u_i \theta}}{\overline{\theta^2}} \frac{D\overline{\theta^2}}{Dt}\frac{1}{2}
    +\underbrace{\frac{1}{2}k \frac{D}{Dt} \left(\frac{\overline{u_i \theta}}{k}\right)+\frac{1}{2} \overline{\theta^2} \frac{D}{Dt} \left(\frac{\overline{u_i \theta}}{\overline{\theta^2}}\right)}_{\simeq 0}
    \end{split}
    \label{WE}
\end{equation}
\end{linenomath}
The same approximation can be used for the molecular diffusion term:
\begin{linenomath}
\begin{equation}
\begin{split}
D_{i\theta}=\frac{1}{2}\frac{\overline{u_i \theta}}{k} D_{k}+\frac{1}{2}\frac{\overline{u_i \theta}}{\overline{\theta^2}} D_{\theta}
    \end{split}
    \label{WE_2}
\end{equation}
\end{linenomath}
and the turbulent diffusion term:
\begin{linenomath}
\begin{equation}
\begin{split}
T_{i\theta}=\frac{1}{2}\frac{\overline{u_i \theta}}{k} T_{k}+\frac{1}{2}\frac{\overline{u_i \theta}}{\overline{\theta^2}} T_{\theta}
    \end{split}
    \label{WE_3}
\end{equation}
\end{linenomath}
Eq. \eqref{WE},\eqref{WE_2} and \eqref{WE_3} lead to the following algebraic balance:
\begin{linenomath}
\begin{equation}
\begin{split}
(P_{k}-\epsilon)\frac{\overline{u_i \theta}}{2k} + (P_{\theta}-\epsilon_{\theta}) \frac{\overline{u_i \theta}}{2\overline{\theta^2}}= P_{\theta i} + \phi_{\theta i} - \epsilon_{\theta i}
    \end{split}
    \label{WE_all}
\end{equation}
\end{linenomath}
where $P_{\theta}$ and $P_k$ indicate the production of thermal variance and turbulent kinetic energy:
\begin{linenomath}
\begin{equation}
    P_{\theta}=-\overline{u_i \theta} \frac{\partial T}{\partial x_i}
    \label{P_t}
\end{equation}
\begin{equation}
    P_{k}=-\overline{u_i u_j} \frac{\partial U_i}{\partial x_j}
    \label{P_k}
\end{equation}
\end{linenomath}
$\epsilon$ and $\epsilon_{\theta}$ are instead the momentum and thermal dissipation rates, respectively:
\begin{linenomath}
\begin{equation}
    \epsilon=\nu \overline{\frac{\partial u_i}{\partial x_j} \frac{\partial u_i}{\partial x_j}}
\end{equation}
\end{linenomath}
\begin{linenomath}
\begin{equation}
    \epsilon_{\theta}=\alpha \overline{\frac{\partial \theta}{\partial x_i} \frac{\partial \theta}{\partial x_i}}
\end{equation}
\end{linenomath}
Figures \ref{residuals} and \ref{WE_plot} represent the application of the weak equilibrium assumption to the DNS data of Kawamura et al.\cite{kawamura2000dns}. Specifically, Figure \ref{WE_plot} compares the transport terms obtained from DNS with those computed by applying eq. \eqref{WE_2} and \eqref{WE_3}. Figure \ref{residuals} represents the residuals of eq. \eqref{FE} and \eqref{WE_all} and compares them with the budget terms $P_{i \theta}$, $\phi_{i \theta}$ and $\epsilon_{i \theta}$. Figure \ref{WE_plot} shows that the weak equilibrium assumption is not perfectly satisfied by the DNS data at both near unity and low Prandtl numbers. The same conclusion was drawn by Vanpouille et al. \cite{vanpouille2013development}, who verified the validity of the weak equilibrium assumption for forced, mixed and natural convection flows: the weak equilibrium hypothesis showed to fail very close to the walls, as well as in regions of vanishing mean velocity gradients. On the other hand, Figure \ref{residuals} clearly shows that assuming weak equilibrium is much better than assuming full equilibrium, as the corresponding residual is lower. Although the weak equilibrium is not satisfied in the near wall region, for near unity Prandtl numbers the peaks achieved by the residuals are significantly lower than the production and redistribution terms. These considerations encouraged the use of this approximation to obtain relatively simple algebraic models \cite{wikstrom2000derivation,so2004explicit,vanpouille2013development}. The diffusion term is instead very important near the wall to produce the correct asymptotic behaviour, and this explains why some authors \cite{dehoux2012algebraic,vanpouille2015development,lecocq2008modelling} altered the balances provided by equations \eqref{FE} and \eqref{WE_all} by using elliptic relaxation (section \ref{EB_sec}). \\
At low Prandtl numbers, the residual computed applying the weak equilibrium hypothesis is of the same order of magnitude of the production term in the near wall region (see Figure \ref{res1}). Therefore, this assumption is less justifiable at low $Pr$, and corrections seem necessary\footnote{The departure from the conditions of weak equilibrium defined by eq.\eqref{WE_all} seems a direct consequence of the lower degree of similarity of thermal and momentum fields, that reduces the correlation of $\overline{u_i \theta}$ with $k$ and $\overline{\theta^2}$.}. \\
Given the algebraic forms indicated by eq.\eqref{FE} and \eqref{WE_all}, the modelling of the redistribution term $\phi_{\theta i}$, which is usually implicit in $\overline{u_i \theta}$, allows to get a complete algebraic model formulation. As in low Prandtl number cases the dissipation is much higher than the redistribution term (see Figure \ref{budgets}), the modelling efforts should be focused on $\epsilon_{i \theta}$, rather than on $\phi_{i \theta}$. \\
It can be noted that the buoyancy production term $\beta g_i \overline{\theta^2}$ and the weak equilibrium assumption introduce the variables $k_{\theta}$ ($k_{\theta}=\overline{\theta^2}/2$) and $\epsilon_{\theta}$ that should be calculated from additional transport equations. Some authors introduced a constant thermal to mechanical time scale ratio ($R$) to get rid of the equation for $\epsilon_{\theta}$:
\begin{linenomath}
\begin{equation}
    R=\frac{k_{\theta} \epsilon}{k \epsilon_{\theta}}
\end{equation}
\end{linenomath}
As shown in Figure \ref{tau}, the assumption of constant $R$ is acceptable far from the wall, and in presence of a wall function approach it will be enough to reasonably predict $\epsilon_{\theta}$. On the other hand, this is not a good approximation in the near wall region, where the time-scale ratio $R$ varies and asymptotically tends to the molecular Prandtl number of the fluid. Probably, the success of the models based on this physically wrong assumption is a result of the compensation job performed by the other calibration parameters contained in the models. \\




   \begin{figure}[h!]
    \centering
%%----start of first subfigure----
    \subfloat[Wall-normal, $Pr=0.71$]{%
        \label{verif}%% label for first subfigure
            \includegraphics[scale=0.35]{figures/WE_final2.eps}
    \hspace{0.02\linewidth}}
%%----start of second subfigure----
    \subfloat[Stream-wise, $Pr=0.71$]{%
        \label{scheme}%% label for second subfigure
      \includegraphics[scale=0.35]{figures/WE_final1.eps}}\\
          \subfloat[Wall-normal, $Pr=0.025$]{%
        \label{verif}%% label for first subfigure
            \includegraphics[scale=0.35]{figures/WE_final4.eps}
    \hspace{0.02\linewidth}}
%%----start of second subfigure----
    \subfloat[Stream-wise, $Pr=0.025$]{%
        \label{scheme}%% label for second subfigure
      \includegraphics[scale=0.35]{figures/WE_final3.eps}}\\
    %\hspace{0.02\linewidth}}
    %%----start of fourth subfigure----
    \caption{Validity of the weak equilibrium assumption for the Kawamura database \cite{kawamura2000dns}. $D_{\theta i}$ and $T_{\theta i}$ calculated from \eqref{WE_2} and \eqref{WE_3} are indicated with solid lines, the corresponding DNS values with dashed lines. The spatial derivatives in eq.\eqref{P_t} and \eqref{P_k} were numerically calculated with finite differences: the uncertainty range related to spatial discretization was estimated using the Richardson extrapolation and indicated with vertical arrows.} %\cite{kawamura2000dns} (dashed lines) compared to those obtained by %applying eq. \ref{WE_all} (solid lines) for Pr=0.71.}
    \label{WE_plot}%% label for entire figure
\end{figure}


   \begin{figure}[h!]
    \centering
%%----start of first subfigure----
    \subfloat[Wall-normal, $Pr=0.71$]{%
        \label{verif}%% label for first subfigure
            \includegraphics[scale=0.33]{figures/eq_4.eps}
    \hspace{0.02\linewidth}}
%%----start of second subfigure----
    \subfloat[Stream-wise, $Pr=0.71$]{%
        \label{scheme}%% label for second subfigure
      \includegraphics[scale=0.33]{figures/eq_3.eps}}\\
          \subfloat[Wall-normal, $Pr=0.025$]{%
        \label{verif}%% label for first subfigure
            \includegraphics[scale=0.33]{figures/eq_2.eps}
    \hspace{0.02\linewidth}}
%%----start of second subfigure----
    \subfloat[Stream-wise, $Pr=0.025$]{%
        \label{res1}%% label for second subfigure
      \includegraphics[scale=0.33]{figures/eq_1.eps}}\\
    %\hspace{0.02\linewidth}}
    %%----start of fourth subfigure----
    \caption{Residuals of eq. \eqref{FE} and \eqref{WE_all} applied to the DNS data of a channel flow at $Re_{\tau}=640$.} %\cite{kawamura2000dns} (dashed lines) compared to those obtained by %applying eq. \ref{WE_all} (solid lines) for Pr=0.71.}
    \label{residuals}%% label for entire figure
\end{figure} 

\subsection{Compensation effects}
The evaluation of the performance of the available thermal turbulence models and their validity range is utmost important to understand limitations and define possible modelling developments. This is not a trivial task, as a thermal turbulence model intrinsically depends on its corresponding momentum turbulence model. If an eddy-viscosity model subjected to the Boussinesq approximation is used for momentum turbulence, it is likely that a thermal model specifically calibrated to work in combination with it tends to overcompensate its errors. Thus, it is rather impossible to evaluate the accuracy of a thermal turbulence model by performing a full RANS simulation, due to the overlap of the uncertainties related to the two turbulence models. In this work, the thermal models considered have been then applied on the basis of fixed DNS momentum fields \cite{kawamura2000dns,oder2019direct,tiselj2012dns} to ensure a meaningful comparison. \\
In what follows, the different approaches adopted to model the turbulent heat flow for near unity and low Prandtl numbers are discussed. The analysis is aided by the results of the application of some of these thermal models to simple flow configurations \cite{kawamura2000dns,oder2019direct,tiselj2012dns} with given momentum fields taken from DNS. 
